HET: Scaling out Huge Embedding Model Training via Cache-enabled Distributed Framework

Embedding models have been an effective learning paradigm for high-dimensional data. However, one open issue of embedding models is that their representations (latent factors) often result in large parameter space. We observe that existing distributed training frameworks face a scalability issue of embedding models since updating and retrieving the shared embedding parameters from servers usually dominates the training cycle. In this paper, we propose HET, a new system framework that significantly improves the scalability of huge embedding model training. We embrace skewed popularity distributions of embeddings as a performance opportunity and leverage it to address the communication bottleneck with an embedding cache. To ensure consistency across the caches, we incorporate a new consistency model into HET design, which provides fine-grained consistency guarantees on a per-embedding basis. Compared to previous work that only allows staleness for read operations, HET also utilizes staleness for write operations. Evaluations on six representative tasks show that HET achieves up to 88% embedding communication reductions and up to 20.68x performance speedup over the state-of-the-art baselines.

==> VLDB2021 Het Accept/convergence.tex <==
Recall that we differ from traditional SSP in the following aspects to improve performance: (1) SSP is not aware of the presence of skew access and provides bounded staleness at the coarse granularity measured by worker clocks, whereas we provide bounded staleness at the fine granularity of individual embedding clocks considering access heterogeneity. (2) SSP assumes a write-through cache so that the server is up-to-date, whereas we adopt a write-back-with-stale server to improve write performance. Given these key differences, we present a new theoretical analysis of the proposed consistency model, instead of reusing that of SSP.
We summarize our proof results showing that our algorithm is guaranteed to converge under our consistency model. The details of the assumptions and proofs are in Appendix A~\cite{hetappendix}.
We decompose the $d$ model parameters into two categories, including the dense parameters $x_0$ and the sparse parameters of $\mathbf{x}_e$ containing $m$ embedding vectors $(x_1, x_2, \ldots, x_m)$. We denote $x_i$ and $\nabla_i f(\mathbf{x})$ as the $i$-th component of $\mathbf{x}$ and $\nabla f(\mathbf{x})$, respectively. Clearly, $\mathbf{x} = (x_0, x_1, \ldots, x_m)$ and $\nabla f = (\nabla_0 f, \nabla_1 f, \cdots, \nabla_m f)$. We have the following theorem:


\begin{theorem}[Global Convergence Rate]
\label{thm:convergence}
  Consider an arbitrary objective function $f$, under the per-embedding-clock-bounded consistency model and and certain assumptions,
  Given the success parameter $\epsilon > 0$, a constant learning rate value 
  \begin{equation}
  \small{\eta \leq \min( \frac{\sqrt{ \epsilon } } {4\sqrt {3}sLMB}, \frac{\sqrt{ \epsilon } } {4\sqrt {L}sMB} , \frac{\epsilon}{ 12 M^2B^2 L})\nonumber}
  \end{equation}
  and  $T = \Theta \left( \frac{ f ( x(0) ) - f_{\text{inf}}}{\epsilon \eta} \right)$ iterations, for worker $j$, we are guaranteed to reach some iterate $\mathbf{x}^j(t^\star)$ with $1 \leq t \leq T$ such that \small{$$\mathbb{E} \| \nabla f(\mathbf{x}^j(t^\star)) \|^2 \leq \epsilon.$$}
\end{theorem}


==> VLDB2021 Het Accept/experiment.tex <==
% \vspace{-2mm}
\section{Experiments}

\paragraph{\textbf{Baselines}} In this section, we compare our prototype system with two state-of-the-art systems: TensorFlow (TF)~\cite{DBLP:conf/osdi/AbadiBCCDDDGIIK16} and Parallax~\cite{DBLP:conf/eurosys/KimYPCJHLJC19}. 
To alleviate the concerns on the difference from the system backbones and implementations, we implement three auxiliary baselines over our system named by \name PS (ASP), \name AR (AllReduce) and \name Hybrid (w/o Cache). 
\name PS follows the ASP algorithm in TensorFlow and each worker pushes its updates to the server without waiting for the others. \name Hybrid keeps the hybrid communication architecture in \name but removes the cache embedding table. 
All of these three baselines are sharing the same computation kernels and communication optimizations (i.e., overlapping, pre-fetching) as \name (denoted by \name Hybrid Cache or \name Cache in the following).

\vspace{-2mm}
\paragraph{\textbf{Datasets and models}}
We select two categories of representative embedding model workloads, including the deep learning recommendation model (DLRM) and the graph neural network (GNN). We use three industrial DLRM models consisting of Wide \& Deep (WDL)~\cite{DBLP:conf/recsys/Cheng0HSCAACCIA16}, DeepFM (DFM)~\cite{DBLP:conf/ijcai/GuoTYLH17} and Deep \& Cross (DCN)~\cite{DBLP:conf/kdd/WangFFW17}. They are evaluated on a popular recommendation dataset, Criteo~\cite{criteo}, which is also the largest standard benchmark in MLPerf~\cite{mlperf}. There could be more than \textit{one trillion model parameters} (i.e., $10^{12}$ floats) from the embedding table when we set $D=4096$ on Criteo.

The second category is GNN~\cite{DBLP:journals/chinaf/GuoQX021,miao2021lasagne,DBLP:conf/kdd/MiaoGZHLMRRSSWW21} model and we select the most popular GraphSAGE~\cite{DBLP:conf/nips/HamiltonYL17} for large graphs. We evaluate on node classification tasks and adopt several graph datasets with different scale: Reddit\cite{hamilton2017inductive}, Amazon\cite{clustergcn} and ogbn-mag\cite{DBLP:conf/nips/HuFZDRLCL20}. More details about the datasets and models are in the Appendix B~\cite{hetappendix}.

\begin{figure}[t]
\centering
\centering
\subfigure[1 Gb cluster]{
\scalebox{1}{
\includegraphics[width=1.0\linewidth]{recepoch6.pdf}
}
\label{fig:recepoch_a}
}
\subfigure[10 Gb cluster]{
\scalebox{1}{
\includegraphics[width=1.0\linewidth]{recepoch7.pdf}
}
\label{fig:recepoch_b}
}
\vspace{-4mm}
\caption{Per epoch time and the speedup of communication time on DLRM tasks.}
\vspace{-4mm}
\label{fig:recepoch}
\end{figure}

\paragraph{\textbf{Experimental setting}}
We implement all of these models in TensorFlow 1.15 and select SGD optimizer with the batch size of 128; the learning rate is selected from [0.001, 0.01, 0.1] by grid search. We have two GPU clusters for our evaluation. In cluster A, each node is equipped with an Nvidia RTX TITAN 24 GB card supporting PCIe 3.0 and 12 GB DRAM for cache (we temporarily improve the DRAM size to 48 GB in the last model scalability experiment). While the servers are in a CPU cluster and each node has two Intel Xeon Gold 5120 CPUs and 376 GB DRAM. The servers and workers clusters are connected by a 1 Gbit Ethernet. Cluster B has similar configurations, but the GPU is replaced by Nvidia V100 and the network is improved to 10 Gbit Ethernet.
The testing AUC thresholds of convergence are set to be around 80\% for the Criteo dataset, as reported in~\cite{DBLP:conf/recsys/Cheng0HSCAACCIA16}. 
For the GNN datasets, due to the customized feature engineering step (e.g., introducing sparse features), we manually set the termination point by predefined values.
All experiments are executed five times, and the averaged results are reported.






\subsection{End-to-end Comparison}
In this section, we first provide end-to-end comparison experiments with the baselines. These experiments are evaluated on 8 workers and 1 remote server. The size of the cache embedding table is set to be 10\% size of the global cache embedding table (listed in Figure~\ref{fig:workload}). We set $D=128$ in the following experiments and tune it in Sec.~\ref{sec:scala}.

\textit{\textbf{Convergence efficiency.}}
Figure~\ref{fig:conv} shows the convergence curves on six different workloads on cluster A. TF PS and HET PS follow the ASP algorithm and cannot converge to the target thresholds in these workloads.
We provide \name with different staleness thresholds $s=10$ and $100$. 
As we can see, our system always outperforms the other baselines on all tasks. When $s=100$, benefited from our cache embedding table mechanism, we could achieve around 4.36-5.14$\times$ speed up compared to \name Hybrid. Compared to $s=10$, it is natural that using a larger $s$ could alleviate more communication costs. The variances regions are quite negligible, which verifies the convergence stability of our methods.
Table~\ref{tab:end2endtime} illustrates the end-to-end convergence time and our \name achieves 6.37-20.68$\times$ speedup compared to TF Parallax. PS-based ASP methods are not listed because they cannot achieve the convergence thresholds. Note that, in our system implementation, we make a unique operation for the keys before the embedding communication operations to avoid redundant embedding transferring costs. However, the GNN-Reddit workload is quite special. It only has node-id embeddings and all embeddings in a mini-batch of data samples are always unique naturally. Therefore, in this case, the costs of unique operation outweigh the benefits, making HET PS ASP slower than TF PS ASP.



\begin{table}[t]
\centering
\small
\caption{End-to-end convergence efficiency comparison.}
\label{tab:end2endtime}
\vspace{-2mm}
\scalebox{0.85}{
\begin{tabular}{l|rrrc}
\toprule 
\makecell{Convergence\\time (h)} & TF Parallax & \name Hybrid & \makecell{\name Cache\\$s=10$} & \makecell{\name Cache\\$s=100$}\\
\midrule 
WDL-Criteo & 56.402 ($\times$10.86) & 26.668 ($\times$5.14) & 9.938 ($\times$1.91) & \textbf{5.193}\\
DFM-Criteo & 27.529 ($\times$9.24) & 13.273 ($\times$4.46) & 5.314 ($\times$1.78) & \textbf{2.978}\\
DCN-Criteo & 99.023 ($\times$11.29) & 42.296 ($\times$4.82) & 17.341 ($\times$1.98) & \textbf{8.770}\\
\midrule
GNN-Amazon  & 8.667 ($\times$20.68) & 1.972 ($\times$4.71) & 0.583 ($\times$1.39) & \textbf{0.419}\\
GNN-Reddit  & 0.752 ($\times$6.37) & 0.514 ($\times$4.36) & 0.123 ($\times$1.04) & \textbf{0.118} \\
GNN-ogbn-mag  & 3.869 ($\times$16.39) & 1.040 ($\times$4.41) & 0.271 ($\times$1.15) & \textbf{0.236}\\
\bottomrule
\end{tabular}}
\vspace{-4mm}
\end{table}


\textit{\textbf{Communication speedup.}}
We also compare the per epoch time on DLRM tasks and provide the following findings. First, through comparative analysis on the per epoch time in Figure~\ref{fig:recepoch_a} and the learning curves in Figure~\ref{fig:conv}, 
we find that \name PS and TF PS follow the same statistical efficiency~\cite{DBLP:conf/sigmod/JiangCZY17} in Figure~\ref{fig:conv} (\name Hybrid and TF Parallax are also the same). Their different convergence speeds come from the backbone optimizations, which verify the correctness of our implementation. Second, PS-based methods often show poor performance compared to hybrid-based methods due to the dense communication. The phenomenon in WDL is not significant because it has fewer dense model parameters than DFM and DCN. Third, these results in Figures~\ref{fig:conv} and \ref{fig:recepoch_a} also imply that existing PS and hybrid communication techniques cannot fundamentally solve the communication bottleneck in large-scale embedding model training. Fortunately, due to the fine-grained caching and consistency, our proposed \name achieves significant performance improvement and up to 88\% ($\approx 1-1/8.2$) embedding communication reduction. Figure~\ref{fig:recepoch_b} shows the per epoch time and communication time speedup comparison on three DLRM tasks under 10 Gbit Ethernet cluster. As shown in Figure~\ref{fig:recepoch_b}, although the speedups are smaller than those in the 1 Gbit Ethernet cluster due to the higher network bandwidth, the communication costs are still the bottleneck of the model training process. We see that our system still outperforms these baselines and achieves up to 2.3$\times$ and 5.2$\times$ speedup compared to HET Hybrid and TF Parallax respectively. Another interesting finding is that HET AR on 1 Gbit Ethernet cluster performs better than HET PS due to the utilization of the PCIe bandwidth cross GPUs. Although AllReduce degenerates to the inefficient AllGather primitive for sparse communication, it still achieves similar performance as HET Hybrid because these baselines involving the PS are suffering from the limited network bandwidth between servers and workers. When we use a 10 Gbit Ethernet, the high network bandwidth significantly improves the speed of PS-based methods. But HET AR maintains similar performance and becomes the slowest among all methods.

\begin{table}[t]
\caption{Final test AUC (\%) with different $s$ on Criteo}
\label{tab:accuracy}
\vspace{-2mm}
\centering
{
\noindent
\renewcommand{\multirowsetup}{\centering}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ccccc|ccc}
\toprule
\textbf{Models}&textbf{$s=0$}&\textbf{$s=100$}&\textbf{$s=10k$}&\textbf{$s=\infty$} & \multirow{2}{*}{ \begin{tabular}[c]{@{}c@{}} \textbf{Cache miss} \\ \textbf{rate (WDL)}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} $s=0$ \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} $s=100$ \end{tabular}} \\
\cmidrule(l){1-5} 
WDL & 79.64 & 79.62 & 78.84 & 74.61 \\
\cmidrule(l){6-8} DFM & 79.74 & 79.73 & 78.96 & 70.91 & 0\% & 80.17\% & 80.15\% \\
DCN & 80.25 & 80.24 & 79.76 & 75.29 & >0\% & 78.17\% & 78.12\%
\\
\bottomrule
\end{tabular}}
\vspace{-2mm}
}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{cache4.pdf}
\vspace{-2mm}
\caption{Cache miss rate under different cache space and strategy settings on GNN tasks.}
\vspace{-2mm}
\label{fig:cache_miss}
\end{figure}

\textit{\textbf{Convergence quality.}}  
We first investigate how much negative impact could the staleness have on the accuracy. We illustrate the convergent model performance (i.e., test AUC) with different staleness thresholds in Table~\ref{tab:accuracy} (left part). 
Due to the inherent robustness of iterative convergent algorithms, we find that our method reaches the target model quality even under moderate
levels of staleness ($s=100$), although the model degradation becomes apparent under high
staleness levels.

We next investigate pathological cases (e.g. is it not possible that prediction with the embedding parameters that are less frequently synchronized may result in less accurate results (i.e., bias)?) We make a further study on the test dataset of Criteo on WDL. As a cache hit (miss) implies the prediction uses stale (up-to-date) embedding parameters, we use cache miss rate to measure the frequency of the prediction using the stale (less frequently synchronized) embedding parameters.
Therefore, we split the test set into two sets based on the cache miss rate. As shown in Table~\ref{tab:accuracy} (right part), the predictions distribution from two models ($s=0$ and $s=100$) are very close, which demonstrates that the stale embeddings will not incur significant predication bias.


\subsection{System Configuration Sensitivity}
We study the impact of different cache embedding table sizes and cache strategy settings. We measure the cache miss rate on GNN task with ogbn-mag and Reddit datasets on cluster A. As shown in Figure~\ref{fig:cache_miss}, LFU often performs a lower cache miss rate than LRU. This is because LFU could reflect the long-term embedding access popularity better. We also evaluate different cache embedding table sizes, including 3\%, 5\%, 10\% and 15\%. As the cache table size growing, the cache miss rate significantly decreases. For ogbn-mag with LFU, given a piece of cache space whose size equals 15\% of the global embedding table size, almost 97\% embedding accesses are performed on the cache embedding table. This experiment strongly verifies the effectiveness of \name and explains how does our cache embedding table help to reduce the communication costs.

\begin{figure}[t]
	\subfigure[WDL-Criteo speedup]{
	    \includegraphics[width=0.47\linewidth]{scala3.png}
	    \label{fig:speedwdl}
	}
	\subfigure[GNN-Reddit speedup]{
        \includegraphics[width=0.47\linewidth]{scala4.png}
        \label{fig:speedreddit}
    }
    \vspace{-4mm}
    \subfigure[WDL-Criteo with different embedding hidden size $D$]{
        \vspace{-2mm}
        \includegraphics[width=0.95\linewidth]{scala_model3.pdf}
        \label{fig:modelwdl}
    }
    %\vspace{-2mm}
    \caption{Scalability study}\label{fig:scala}
    \vspace{-4mm}
\end{figure}

% \vspace{-2mm}
\subsection{Scalability}
\label{sec:scala}
We conduct a scalability study in terms of run time speedup on cluster A over 4 servers with 1, 2, 4, 8, 16, and 32 workers respectively. As shown in Figure~\ref{fig:speedwdl} and Figure~\ref{fig:speedreddit}, both TF PS and TF Parallax have limited scalability suffering from large amounts of embedding communication costs. By contrast, our \name achieves improved scalability by caching the hot embeddings. We also note that all methods show better scalability on GNN-Reddit than WDL-Criteo. Because the latter has a larger embedding table and becomes more communication-intensive and more difficult to scale up. 
We also study the model scalability of \name on WDL-Criteo by increasing the embedding size $D$ up to 4096 (around \textit{one trillion model parameters}) over 32 workers. Figure~\ref{fig:modelwdl} shows that \name significantly outperforms TF and Parallax since their PS architecture faces a more serious communication bottleneck with such a large scale embedding table.

